VERT: Verified Equivalent Rust Transpilation with Large Language Models as Few-Shot Learners

Rust is a programming language that combines memory safety and low-level control, providing C-like performance while guaranteeing the absence of undefined behaviors by default. Rust's growing popularity has prompted research on safe and correct transpiling of existing code-bases to Rust. Existing work falls into two categories: rule-based and large language model (LLM)-based. While rule-based approaches can theoretically produce correct transpilations that maintain input-output equivalence to the original, they often yield unreadable Rust code that uses unsafe subsets of the Rust language. On the other hand, while LLM-based approaches typically produce more readable, maintainable, and safe code, they do not provide any guarantees about correctness. In this work, we present VERT, a tool that can produce readable Rust transpilations with formal guarantees of correctness. VERT's only requirement is that there is Web Assembly compiler for the source language, which is true for most major languages. VERT first uses the Web Assembly compiler to obtain an oracle Rust program. In parallel, VERT uses an LLM to generate a readable candidate Rust program. This candidate is verified against the oracle, and if verification fails, we regenerate a new candidate transpilation until verification succeeds. We evaluate VERT by transpiling a suite of 1,394 programs taken from competitive programming style benchmarks. Combining Anthropic's Claude-2 and VERT increases Rust transpilations passing property-based testing from 31% to 54% and bounded model-checking from 1% to 42% compared to using Claude alone. In addition, we evaluate VERT's ability to generate non-trivial safe Rust on programs taken from real-world C projects that make significant use of pointers. Our results provide insights into the limitations of LLMs to write safe Rust.

==> sections/limitations.tex <==
\section{Limitations}

\subsection{Limitations of the Equivalence Checking}
\tool's equivalence checking is performed in 3 stages with increasing
guarantees: PBT, bounded, and full verification. The first 2 phases do
not provide any exhaustive guarantees. The quality of PBT depends
heavily on the inputs generated, and thus the seed used to generate
the random inputs. Bounded verification may miss bugs or divergences
in LLM and \rwasm-generated programs if they occur beyond the loop
unwinding bound. Full verification provides exhaustive guarantees but
few programs actually reach that stage due to performance limitations
of Kani. We posit that these limitations will be mitigated with future
improvements to Kani.

\subsection{Trusted Computing Base}
The Trusted Computing Base (TCB)~\cite{rushby_tcb_1981} is the set of
all software and hardware the user must trust in order to trust the
result of the full verification. We note that \tool has a large TCB
compared to traditional formal verification frameworks like
Coq~\cite{coquand_constructions_1985} or
Isabelle/HOL~\cite{nipkow_isabellehol_2002}. To trust the results of
\tool, the user must trust Kani, its CBMC backend, the original
language's Wasm compiler, \rwasm, the Rust compiler, and all of the
transitive dependencies of the respective software. We posit that this
TCB is still more trustworthy and easily checked than the LLM.

